Low Resourced Machine Translation via Morpho-syntactic Modeling: The Case of Dialectal Arabic

We present the second ever evaluated Arabic dialect-to-dialect machine translation effort, and the first to leverage external resources beyond a small parallel corpus. The subject has not previously received serious attention due to lack of naturally occurring parallel data; yet its importance is evidenced by dialectal Arabic's wide usage and breadth of inter-dialect variation, comparable to that of Romance languages. Our results suggest that modeling morphology and syntax significantly improves dialect-to-dialect translation, though optimizing such data-sparse models requires consideration of the linguistic differences between dialects and the nature of available data and resources. On a single-reference blind test set where untranslated input scores 6.5 BLEU and a model trained only on parallel data reaches 14.6, pivot techniques and morphosyntactic modeling significantly improve performance to 17.5.

==> 7-Results.tex <==
To verify the usefulness of phrase pivoting and the additional benefit of adding morpho-syntactic constraints to the \textsc{DIR+PP} system, we evaluated our \textsc{Direct}, \textsc{DIR+PP}, and Direct + Phrase Pivot with Morpho-syntactic Features (\textsc{DIR+PP+MORPH}) systems on a 2,000 sentence blind test set from our BTEC corpus. As shown in Table \ref{FinalResultsTable}, our findings on the development set were confirmed on the blind test, where all improvements were statistically significant.


\begin{table}[tbh]
\normalsize
%\setlength{\tabcolsep}{0pt}
\centering
%\begin{footnotesize}
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Model} & \textbf{Dev} & \textbf{Dev OOV} & \textbf{Test} & \textbf{Test OOV} \\ \hline
No-Translation & 6.48 & 100 & 6.45 & 100 \\ \hline
Direct & 15.44 & 4.6 & 14.61 & 5.4 \\ \hline
DIR+PP & 17.41 & 0.9 & 16.69 & 1.0 \\ \hline
\textbf{DIR+PP+MORPH} & \textbf{18.03} & 0.9 & \textbf{17.48} & 1.0 \\ \hline
\end{tabular}
%}
\caption{Comparing BLEU scores of systems with and without morpho-syntactic features on development and blind test sets. Out-of-Vocabulary rates are reported as percentages.}
\label{FinalResultsTable}
%\end{footnotesize}
\end{table}

%\begin{table}[]
%\setlength{\tabcolsep}{2pt}
%\centering
%\begin{footnotesize}
%\begin{tabular}{|l|l|l|}
%\hline
%\textbf{Model} & \textbf{BLEU on Dev} & \textbf{BLEU on Test} \\ \hline
%Direct & 15.44 & 14.61 \\ \hline
%Direct + Phrase Pivot & 17.41 & 16.69 \\ \hline
%\begin{tabular}[c]{@{}l@{}}Direct + Phrase Pivot with\\ Morpho-Syntactic Constraints\end{tabular} & 18.03 & 17.48 \\ \hline
%\end{tabular}
%\caption{Comparing the performance of models with and without morpho-syntactic features on development and blind test sets.}
%\label{FinalResultsTable}
%\end{footnotesize}
%\end{table}

==> 9-DiscussionAndFutureWork.tex <==
%Additionally, there is a wealth of literature on generating comparable corpora which can provide a powerful boost to MT systems in the absence of sufficient true parallel data. The process typically consists of using meta data such as publish dates to identify documents which could potentially contain similar content \citep{resnik2003web}. Then such documents are searched for candidate parallel sentences, usually using word overlap scores based on words known to be good translations of one another from a seed lexicon and/or parallel data \citep{munteanu2005improving}. Max et al. \cite{max2012generalizing} and Cettolo et al. \cite{cettolo2010mining} look for parallelism at the sub-sentential level, which is critical when even monolingual data is sparse as this increases the amount of comparable data that can be extracted. Once the search space is reduced to a tractable number of candidate sentences (or phrases), features are learned using the seed data and Expectation Maximization is performed to identify the candidate sentences most likely to be parallel. This process can be iterated as in Dong et al. \cite{dong2015iterative} by appending the comparable sentences identified via Expectation Maximization to the seed parallel data and repeating the process. Fung and Cheung \cite{fung2004mining} also demonstrate that this process can be successful even when the monolingual corpora in the source and target language are far from comparable.

%%%%%%%%%%%%%%


Given that many DA pairs may not have pivot data available, the most pressing future work is to develop a dialect-agnostic tokenizer and analyzer which does not suffer from the Egyptian bias that ours does.
This will reduce data sparsity regardless of the nature of the low-resourced MT settings for any DA pair, and it will enable better morpho-syntactic modeling.

Additionally, improving on the dialect identification work of \cite{zaidan-callisonburch:2011:ACL-HLT2011}, \cite{Diab_10_LREC}, and \cite{elfardy-diab:2013:Short} will enable us to collect more monolingual data for language modeling. 
Modeling syntactic variation in DA is critical as word order varies considerably.
In Egyptian and Levantine for instance, adjective-adverb order is often flipped, e.g., `very pretty' in Egyptian, <^gmyl qwy> \textit{jmyl qwy}, with the adverb following the adjective, becomes <ktyr .hlw> \textit{ktyr Hlw} in Levantine, with the adverb first.
The same occurs with demonstrative/article-noun order, as `today' in Egyptian, <Alnhrdh>  \textit{Alnhr-dh}, literally, `day-this', becomes <Alywm> \textit{Al-ywm} in Levantine, literally, `the-day'.
Were a Levantine speaker to use a demonstrative to modify the same noun, it would also come before the noun, unless used for emphasis.
Gaining more data for language modeling via dialect identification would allow such phenomena to be modeled more accurately.

This additional monolingual data can also be mined for comparable sentences to augment the parallel training set. This typically involves using metadata \citep{resnik2003web} and seed data \citep{munteanu2005improving} to identify pairs of related sentences or phrases in the source and target languages \citep{max2012generalizing,cettolo2010mining}.
These are then iteratively classified via expectation maximization with phrases identified as parallel being added to the seed data \citep{dong2015iterative}.
Models trained thusly produce noisy phrase pairs, often imperfectly modeling morpho-syntactic property sets.
Thus, the same morpho-syntactic constraints that improved \textsc{DIR+PP+MORPH} can be adapted to improve MT via comparable corpora. 

%The \textsc{Synthetic} model has already demonstrated that noisy pseudo-parallel data can improve results, though we are unsure if further work in this direction will be fruitful. We recreated the model using \textsc{DIR+PP+MORPH} to fabricate parallel data instead of \textsc{Direct}, however, this did not improve performance. Before investing in other solutions, it might be worth investigating why the \textsc{Direct} \textsc{Synthetic} model taught itself to fix its mistakes whereas the \textsc{DIR+PP+MORPH} \textsc{Synthetic} model reinforced its own errors.
